Quadratic number fields with unramified $SL_2(5)$-extensions

Continuing the line of thought of an earlier work, we provide the first infinite family of quadratic number fields with everywhere unramified Galois extensions of Galois group $SL_2(5)$, the (unique) smallest nonsolvable group for which this problem was previously open. Our approach also improves upon previous work by yielding the first infinite family of real-quadratic fields possessing an unramified Galois extension whose Galois group is perfect and not generated by involutions. Our result also amounts to a new existence result on quintic number fields with squarefree discriminant and additional local conditions.

==> sl25_unram_anc.tex <==
//Magma code for calculations relevant for the proof of the main theorem:


// ***** 1) Determination of values a=a(w) and c=c(w) such that F(s,x):=x^3*(x-1)^2-c*s^2*(x-a) has desired decomposition groups at branch points

k<a>:=FunctionField(Rationals());
p<t>:=PolynomialRing(k);
q<x>:=PolynomialRing(p);
f:=x^2*(x-1)^3-t*(x-a);
fac:=Factorization(Discriminant(f));
g:=fac[2][1]; //the quadratic factor of the discriminant, corresponding to the two non-zero finite branch points
k2<b>:=FunctionField(t^2-(a^2-22/25*a+1/25)); //root field of the discriminant of g
p<t>:=PolynomialRing(k2);q<x>:=PolynomialRing(p);
f:=t^2*(t-1)^3-Roots(p!g)[1][1]*(t-a);
t0:=Roots(p!g)[1][1];
fac:=Factorization(f);
h:=fac[2][1]; //the cubic factor of x^2(x-1)^3-t0*a; its splitting field is the residue extension over t0
dh:=Discriminant(h); 
dh*t0;

p<c,y>:=PolynomialRing(k,2);
/* Now write out equations for dh*t0 =: u*b+v = c*(y*b+1) with u,v in Q(a) given by above expression for t0 and c,y in Q(a) to be determined*/

j:=ideal<p|
c*2*y-(1220703125/262144*a^9 - 6787109375/262144*a^8 + 3904296875/65536*a^7 -
    4761015625/65536*a^6 + 6508484375/131072*a^5 - 2392131125/131072*a^4 +
    195981795/65536*a^3 - 5441985/65536*a^2 - 1483515/262144*a - 98415/262144), c*(y^2*(a^2-22/25*a+1/25)+1) - (- 1220703125/262144*a^10 + 3662109375/131072*a^9 - 18509765625/262144*a^8 +
    3179453125/32768*a^7 - 10202278125/131072*a^6 + 2367172125/65536*a^5 -
    1158713365/131072*a^4 + 27959445/32768*a^3 + 145071/262144*a^2 +
    40095/131072*a + 19683/262144)>;
gb:=GroebnerBasis(j);

F:=gb[#gb];
F*:=Lcm([Denominator(u): u in Coefficients(F)]); //equation for curve parameterizing admissible values for y in terms of a
F;

p<a,y>:=PolynomialRing(Rationals(),2);
cc:=Curve(AffineSpace(p),(a^10 - 134/25*a^9 + 7461/625*a^8 - 221704/15625*a^7 + 748426/78125*a^6 -
    34970148/9765625*a^5 + 158757346/244140625*a^4 - 9140936/244140625*a^3 -
    66339/244140625*a^2 - 4374/244140625*a + 729/244140625)*y^2 + (2*a^9 -
    246/25*a^8 + 12312/625*a^7 - 318728/15625*a^6 + 890652/78125*a^5 -
    31260996/9765625*a^4 + 3316952/9765625*a^3 + 17496/48828125*a^2 +
    1458/9765625*a + 1458/48828125)*y + a^8 - 112/25*a^7 + 4972/625*a^6 -
    21904/3125*a^5 + 241678/78125*a^4 - 5647568/9765625*a^3 + 172044/9765625*a^2
    + 11664/9765625*a + 729/9765625); Genus(cc);
    /* Genus 0 curve, so in the following, can find parameter w via standard Riemann-Roch space computation.
    */
    
pt:=cc![0,-5];
pl:=Places(pt);
Degree(pl[1]);
rrs,phi:=RiemannRochSpace(Divisor(pl[1]));
MinimalPolynomial(phi(Basis(rrs)[1]));

/* Now have parameterization a=a(w), which can be evaluated in above GroebnerBasis calculation to also determine c.
    After some simplifying parameter transformations, reach parameterization a=2*w^2 
   */
k<w>:=FunctionField(Rationals());
p<a>:=PolynomialRing(k);
w:=(2^12*3^3/w-14385);
f:=a*w^2 + 28770*a*w + (206928225*a - 24461180928); //minimal polynomial found above
a:=Roots(f)[1][1];a;  //yields a=2w^2

// Now redo Groebner basis calculation to find c=c(w)
k<w>:=FunctionField(Rationals());
a:=2*w^2;
p<c,y>:=PolynomialRing(k,2);
j:=ideal<p|
c*2*y-(1220703125/262144*a^9 - 6787109375/262144*a^8 + 3904296875/65536*a^7 -
    4761015625/65536*a^6 + 6508484375/131072*a^5 - 2392131125/131072*a^4 +
    195981795/65536*a^3 - 5441985/65536*a^2 - 1483515/262144*a - 98415/262144), c*(y^2*(a^2-22/25*a+1/25)+1) - (- 1220703125/262144*a^10 + 3662109375/131072*a^9 - 18509765625/262144*a^8 +
    3179453125/32768*a^7 - 10202278125/131072*a^6 + 2367172125/65536*a^5 -
    1158713365/131072*a^4 + 27959445/32768*a^3 + 145071/262144*a^2 +
    40095/131072*a + 19683/262144)>;
gb:=GroebnerBasis(j);
j:=ideal<p|j, Factorization(gb[#gb])[1][1]>;
c:=-Evaluate(GroebnerBasis(j)[1],[0,0]);
num:=Numerator(c);
denom:=Denominator(c);
lc:=LeadingCoefficient(Numerator(c));
Factorization(num);
Factorization(denom);
Factorization(Numerator(lc));
Factorization(Denominator(lc));

/* Now cancellation of squares out of c gives the claimed form c=c(w)=-2*(50*w^2-27)*(10*w^2+8*w+1)*/   
   
   
   
   
   
   
   
   
   
   
   
   
  // ********** 2) Check for numbers of real roots in different segments of punctured real line, for varying values of parameter w :
  
  p<w>:=PolynomialRing(Integers());
q<t>:=PolynomialRing(p);
q2<x>:=PolynomialRing(q);
f:=x^2*(x-1)^3+2*t^2*(50*w^2-27)*(10*w^2+8*w+1)*(x-2*w^2);
d:=Discriminant(f);
lc:=LeadingCoefficient(d);
fac:=Factorization(lc);
r:=[rr[1]: rr in Roots(PolynomialRing(RealField())!&*[a[1]: a in fac])];
e:=Discriminant(&*[a[1]: a in Factorization(d)]);
e2:=&*[a[1]: a in Factorization(e)];
for rr in Roots(PolynomialRing(RealField())!e2) do if not rr[1] in r then Append(~r, rr[1]); end if; end for;
r:=Sort(r);r;

test:=[BestApproximation(r[1]-1, 10^6)]; 
for j:=1 to #r-1 do Append(~test,BestApproximation((r[j]+r[j+1])/2,10^6)); end for;
Append(~test, BestApproximation(r[#r]+1, 10^6)); test;

for w in test do
p<t>:=PolynomialRing(Rationals());
q<x>:=PolynomialRing(p);
f:=x^2*(x-1)^3+2*t^2*(50*w^2-27)*(10*w^2+8*w+1)*(x-2*w^2);
d:=Discriminant(f);fac:=Factorization(d);
s:=[rr[1]: rr in Roots(PolynomialRing(RealField())!&*[a[1]: a in fac])];
s2:=[s[1]-1];
for j:=1 to #s-1 do Append(~s2, (s[j]+s[j+1])/2); end for;
Append(~s2, s[#s]+1);
for t0 in s2 do x:=t; #Roots(PolynomialRing(RealField())!(x^2*(x-1)^3+2*t0^2*(50*w^2-27)*(10*w^2+8*w+1)*(x-2*w^2)));
end for;
<w*1.0>; end for;










// *********** 3) Calculation of discriminants relevant for the proof of Theorem 3.2 and Corollary 3.3:

/*3a) mod-4 calculation of discriminant of f_{s,w}(X). The first two cases simply yield the result  "1 mod 4"; for the third case (w1 and w2 odd), we give two options, which are both odd and differ by 2. */

p<u1,u2>:=PolynomialRing(Integers(),2);
q<x>:=PolynomialRing(p);
w1:=2*u1+1; w2:=2*u2; s1:=1;s2:=4; 
/*due to clearing of denominators in below polynomial, this corresponds to specialization f_{w1/w2, 1/4*w2^3}(X) in notation of the proof of Thm.3.2*/
f:=s2^2*x^2*(x-1)^3-2*s1^2*(-50*w1^2+27*w2^2)*(10*w1^2+8*w1*w2+w2^2)*(w2^2*x-2*w1^2);
d:=Discriminant(f);
fac:=Factorization(d);
d:=Sign(LeadingCoefficient(d))*&*[a[1]: a in fac| a[2] mod 2 ne 0]; 

p0:=PolynomialRing(Integers(4),2);
d0:=p0!d;
d0; 

p<u1,u2>:=PolynomialRing(Integers(),2);
q<x>:=PolynomialRing(p);
w1:=2*u1; w2:=2*u2+1; s1:=2;s2:=1;
f:=s2^2*x^2*(x-1)^3-2*s1^2*(-50*w1^2+27*w2^2)*(10*w1^2+8*w1*w2+w2^2)*(w2^2*x-2*w1^2);
d:=Discriminant(f);
//d;
fac:=Factorization(d);
d:=Sign(LeadingCoefficient(d))*&*[a[1]: a in fac| a[2] mod 2 ne 0]; 

p0:=PolynomialRing(Integers(4),2);
d0:=p0!d;
d0;

p<u1,u2>:=PolynomialRing(Integers(),2);
q<x>:=PolynomialRing(p);
w1:=2*u1+1; w2:=2*u2+1; for s1 in [2,6] do s2:=1;
f:=s2^2*x^2*(x-1)^3-2*s1^2*(-50*w1^2+27*w2^2)*(10*w1^2+8*w1*w2+w2^2)*(w2^2*x-2*w1^2);
d:=Discriminant(f);
fac:=Factorization(d);
d:=Sign(LeadingCoefficient(d))*&*[a[1]: a in fac| a[2] mod 2 ne 0]; 
p0:=PolynomialRing(Integers(4),2);
d0:=p0!d;
<s1,s2,d0>; end for;

    

// 3b) Now discrimnant calculations relevant for Cor.3.3:
p<s>:=PolynomialRing(Integers());
q<x>:=PolynomialRing(p);
f:=x^2*(x-1)^3-86*s^2*(9*x-8);
d:=Discriminant(f); 
fac:=Factorization(d);
d2:=Discriminant(&*[a[1]: a in fac]);
PrimeDivisors(120*LeadingCoefficient(d)*d2); // These are the ``exceptional primes" needing extra treatment

f0:=x^2*(x-1)^3-86*(86*s^3)^2*(9*x-8);
d3:=Discriminant(f0);
Sign(d3); Factorization(d3); // determining the quadratic subfield of the S5-extension cut out by f0
    

